SaludConectaMX: Lessons Learned from Deploying a Cooperative Mobile Health System for Pediatric Cancer Care in Mexico

We developed SaludConectaMX as a comprehensive system to track and understand the determinants of complications throughout chemotherapy treatment for children with cancer in Mexico. SaludConectaMX is unique in that it integrates patient clinical indicators with social determinants and caregiver mental health, forming a social-clinical perspective of the patient's evolving health trajectory. The system is composed of a web application (for hospital staff) and a mobile application (for family caregivers), providing the opportunity for cooperative patient monitoring in both hospital and home settings. This paper presents the system's preliminary design and usability evaluation results from a 1.5-year pilot study. Our findings indicate that while the hospital web app demonstrates high completion rates and user satisfaction, the family mobile app requires additional improvements for optimal accessibility; statistical and qualitative data analysis illuminate pathways for system improvement. Based on this evidence, we formalize suggestions for health system development in LMICs, which HCI researchers may leverage in future work.

==> 2_Background.tex <==
\section{Background}

Telehealth tools serve as \textit{supplementary} resources to complement in-person clinic visits and effectively address diverse patient needs \cite{gajarawala2021telehealth}, especially for those in under-served areas \cite{romain2022effect}; by using virtual platforms, patients in low-income and remote regions can receive prompt consultations, mitigating outcome discrepancies across socioeconomic backgrounds \cite{barwise2023perceptions}. These tools help bridge health gaps by improving healthcare access, alleviating financial and transportation burdens, enhancing health education and awareness, addressing cultural and linguistic sensitivities, and offering culturally relevant interfaces \cite{riley2012health}. They also promote the adoption of digital health records and standardized protocols, facilitating smooth information exchange among various healthcare facilities, thereby enhancing continuity of care and associated clinical decision-making \cite{haleem2021telemedicine}. %Although these systems may sometimes create barriers for collecting important medical data (e.g., vitals, labs), as well as give rise to certain legal and regulatory hurdles, patient privacy concerns \cite{gajarawala2021telehealth}, the anticipated benefits most often outweigh these cons. 
%Implementing a telehealth tool for chronic diseases like cancer, especially in pediatric patients from LMICs, can enhance real-time data flow between healthcare providers and caregivers, informing decisions that minimize the risk of complications during treatment cycles, which can save lives and reduce financial burden for both health systems and families \cite{lall2018models}. 

While evidence shows that telehealth systems were successfully implemented during the COVID-19 pandemic in LMICs like India, China, Brazil, and Pakistan \cite{GlobalBurden}, to our knowledge, none facilitate the care of children with cancer, especially those at risk of developing complications after treatment. At the same time, within the HCI community, several interventions and research studies have been conducted in related areas like breast cancer \cite{Jacobs2016, Jacobs2018}, and chronic illnesses \cite{Jacobs2019} more generally. However, these are focused on adult patients living outside of LMIC contexts. Previous HCI research on designing technologies for childhood cancer, specifically, has primarily focused on promoting positive experiences during treatment \cite{Choi2020}, as well as identifying and supporting patient needs within the parent-child dyad \cite{Seo2021}. While pediatric cancer care coordination using communication technologies has been studied \cite{Nikkhah2022}, this work focuses more on balancing role responsibilities and tasks within families, rather than supporting patient monitoring between caregivers and healthcare providers. To the best of our knowledge, no comprehensive tool has been implemented toward this end. Therefore, in this work, we develop a system specifically catered to the needs of pediatric cancer patients and their care teams, which consist of both healthcare professionals and families.%, incorporating the specific socioclinical conditions that may impact their health risks and associated medical decisions.

%- interviewing children with cancer to inform health technologies \cite{Choi2020}
%-interviews to identify challenges around parent-child communication for illness management \cite{Seo2021}

%We situate our work by providing an overview of the current health system challenges in Mexico. We also synthesize previous work in HCI on telehealth systems.

%\subsection{Cancer Occurrence \& Healthcare Access in Mexico}

%More than two-thirds of the world’s cancers are projected to occur in LMICs by 2024 \cite{GlobalBurden}. On top of this, the fragmentation of health services in LMICs generates delays in the diagnosis and treatment of children with cancer, reducing chances of survival \cite{siqueira2021impacts}. In Mexico, a middle-income country with approximately $44,697,145$ youth between $0-19$ years old, the national incidence of cancer rates are reported as $111.4$ cases per one million for children $0-9$ years old and $68.1$ for children $10-19$ years old, with the highest incidence of $135.8$ per one million for children $0-4$ years old \cite{mohar2017cancer}. Meanwhile, Mexico faces significant changes in the health system. For exmaple, over $56\%$ of youth do not have access to any type of social security program \cite{stat2019}. With the dismantling of Seguro Popular, a universal coverage program, and the elimination of social programs focused on vulnerable populations, healthcare for children with cancer becomes a topic of interest due to the demand for tertiary care; significant delays in diagnosis and treatments have been well documented in vulnerable groups of the population, like rural and suburban contexts \cite{knaul2023setbacks}. Hospital A offers medical care to children from families without social protection, providing treatment and medical care mainly to children with cancer from the central and southern areas of the Mexican territory, making this institution a relevant context for this work.


%\subsection{Existing Gaps in HCI for Telehealth}%{HCI Contributions toward Designing Telehealth Solutions for LMICs}
%Over a decade ago, a study was puublished reflecting on avenues for technology-supported collaborative healthcare work \cite{}, arguing for further development of socio-technical systems with patient-centered focuses across multiple settings and roles. 
%The HealthApp-MD system fills two existing gaps within telehealth tools: (1) it supports an under-served patient population (pediatric cancer patients) and (2) it provides the care team with continuous support in assessing the child's social and clinical condition over time (collaborative monitoring to supplement in-person healthcare). While evidence shows that telehealth systems were successfully implemented during the pandemic in LMICs like India, China, Brazil, and Pakistan \cite{GlobalBurden}, to our knowledge, none facilitate the care of children with cancer, especially those at risk of developing complications after treatment. At the same time, within the Human-Computer Interaction (HCI) community, several interventions and research studies have been conducted in related areas like breast cancer \cite{Jacobs2016, Jacobs2018}, and chronic illnesses \cite{Jacobs2019} more generally. However, these are focused on adult patients living outside of LMIC contexts. Therefore, in this work, we develop a system specifically catered to the needs of pediatric cancer patients and their care teams, incorporating the specific socioclinical conditions that may impact their health risks and associated medical decisions.

%Telehealth tools address many challenges regarding healthcare access for under-served communities, but the drawbacks of these systems can often impact aspects of care \cite{gajarawala2021telehealth}. For example, many telehealth tools are used to replace in-person health visits, which result in impersonal online interactions. Additionally, these online interactions create barriers for collecting important medical data (e.g., vitals, labs) and often produce incomplete medical records. Other challenges include legal and regulatory hurdles, patient privacy concerns, and delays in medical care. Unlike many of the existing telehealth technologies, the HealthApp-MD system \textit{supplements} but does not replace in-person care. The caregiver is able to collaborate with the medical team on monitoring the child's health conditions, providing information about the child's symptoms and social factors as they evolve over time. 



%Previous research has outlined strategies for 
%Additionally, overcoming barriers such as insufficient awareness and acceptance of screening programs, sociocultural factors, limited symptom knowledge, social stigma, costs, and familial obligations are essential for the successful design and implementation of telehealth tools within private contexts \cite{sullivan2021cancer}. 

==> 5_Results.tex <==
\section{Findings}

==> 6_Discussion.tex <==
\section{Discussion}
%\subsection{Limitations and Future Research}
SaludConectaMX is a friendly and flexible tool that facilitates collaboration between the clinical team and the primary caregiver of children with cancer. Its novelty stems from the integration of clinical, caregiver, and SDOH dimensions to capture a child’s holistic health picture, as it evolves throughout cancer treatment. SaludConectaMX also offers the opportunity to provide a comprehensive classification of risk to patients with a broader understanding of their context. Throughout its pilot deployment, the system has demonstrated high hospital usage rates, user satisfaction, iterative improvements, and opportunities for future work. 

The successful design and implementation of this tool are not without challenges and limitations. Pre-existing conditions, such as a lack of key infrastructure, was a major barrier to system development and deployment; web access was often limited both within the Hospital $H$nd patient residences and/or communities. This limitation persists in both settings and continues to impact data collection and communication opportunities, echoing the literature \cite{schwalbe2020artificial}. Furthermore, certain hospital services used a commercial electronic system prior to the integration of SaludConectaMX, while other critical services throughout the hospital maintain a dependency on paper files. Therefore, the integration of SaludConectaMX extends data collection to an additional modality. However, we anticipate that the beneficial impacts of our system (i.e., future risk prediction, potential financial savings, etc.) will outweigh these complexities long-term. 

Other challenges associated with this work pertained to system changes, time constraints, and documentation burden. The pilot phase system underwent multiple system changes, reducing the time available to implement the tool and resolve the needs of Hospital $H$ and their patients. Meanwhile, documentation time, particularly for caregivers, is limited by their availability as they attend to patients, as well as their backgrounds and circumstances (e.g., health literacy, digital literacy, web access, etc.). For these reasons, the family mobile application will require additional work to make this aspect of the system both useful and manageable for caregivers, as the intention of the application is to benefit the patient without overburdening their loved ones. For instance, caregivers may perceive immediate benefit from a system with more interactivity and dynamic, helpful feedback, such that documentation energy does not feel wasted. System improvements will focus more intently on caregiver expectations and needs. 

Although challenges remain, the implementation of SaludConectaMX creates opportunities for future work. Throughout the pilot phase, new evidence emerged regarding patients with multiple caregivers who possessed various roles surrounding attention, food, medical supplies, and financing. It became evident that the families’ social networks may impact the patients’ health risks, especially as their support systems evolve over time, and data collection should capture these elements. Another important (related) aspect involves the information recorded in free-form notes by hospital staff, which often contain information related to cultural behaviors, care barriers, financial concerns, social networks, and additional clinical data that the existing form fields fail to capture. As a result, future work will incorporate useful feature extraction via text mining and language modeling techniques to account for these components. Finally, using the data collected across the system, we plan to build comprehensive models that classify patients into high-risk and low-risk groups for adverse outcomes throughout the patient trajectory. Once validated, these models may be integrated into the SaludConectaMX system to facilitate decision-making among the patients’ care team and make a tangible impact on human lives. 


==> old_tables.tex <==
\iffalse
\captionsetup{width=.48\textwidth}

\begin{table*}[h]
  \begin{minipage}{.5\linewidth}
    \centering
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}c@{}}Form Name\\\end{tabular}}          & \textbf{\begin{tabular}[c]{@{}c@{}}Completion Time\\\end{tabular}}                                                         & \textbf{N} & \textbf{\begin{tabular}[c]{@{}c@{}}Completed at \\ least once (\%)\end{tabular}} \\ \hline
\rowcolor[HTML]{FFFFFF} 
Medical History (HWA)                                                 & Enrollment (1x)                                                                                                             & 274        & \cellcolor[HTML]{57BB8A}274 (100\%)                                              \\ \hline
\rowcolor[HTML]{FFFFFF} 
Social Work (HWA)                                                     & \begin{tabular}[c]{@{}c@{}}Enrollment \\ (plus annually)\end{tabular}                                                       & 274        & \cellcolor[HTML]{A1C77A}250 (95.1\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
SDOH (HWA)                                                            & Enrollment (1x)                                                                                                             & 274        & \cellcolor[HTML]{90C57D}253 (96.2\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Oncology (HWA)                                                        & Oncology Appts.                                                                                                             & 274        & \cellcolor[HTML]{93C57D}263 (96.0\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}c@{}}Caregiver \\ Burden (FMA)\end{tabular}                                                         & Enrollment (1x)                                                                                                             & 274        & \cellcolor[HTML]{F8BC6A}171 (62.4\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}c@{}}Caregiver \\ Stress (FMA)\end{tabular}                                                         & Enrollment (1x)                                                                                                             & 274        & \cellcolor[HTML]{F8BE6A}175 (63.9\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}c@{}}Caregiver \\ Depression (FMA)\end{tabular}                                                     & Enrollment (1x)                                                                                                             & 274        & \cellcolor[HTML]{F8BE6A}175 (63.9\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}c@{}}Caregiver \\ Substance Use (FMA)\end{tabular}                                                   & Enrollment (1x)                                                                                                             & 274        & \cellcolor[HTML]{F8BE6A}175 (63.9\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
SDOH (FMA)                                                            & Oncology appts.                                                                                                             & 274        & \cellcolor[HTML]{F6B86B}158 (57.7\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
S\&S (FMA)                                                            & Every 8 Hours                                                                                                               & 274        & \cellcolor[HTML]{F7BB6A}165 (60.2\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Emergency (HWA)                                                       & \begin{tabular}[c]{@{}c@{}}Emergency Visits\\ (hospitalization day 1)\end{tabular}                                          & 274        & \cellcolor[HTML]{C0C0C0}169 (61.7\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Infectiology (HWA)                                                    & \begin{tabular}[c]{@{}c@{}}At least once during\\ hospitalizations \\ (+ optional during\\  oncology appts.)\end{tabular}   & 169        & \cellcolor[HTML]{A7C879}160 (94.7\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}c@{}}Clinical Alarm \\ Signs (HWA)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Days 1 and 3 of \\ hospitalizations\\ (+ optional during\\  oncology appts.)\end{tabular}        & 169        & \cellcolor[HTML]{F7D567}151 (89.3\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
S\&S (HWA)                                                            & \begin{tabular}[c]{@{}c@{}}Every 6 hours during\\ Oncology appts. \&\\ Every 4 hours during\\ hospitalizations\end{tabular} & 169        & \cellcolor[HTML]{B9CB75}158 (93.5\%)                                             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Outcomes (HWA)                                                        & \begin{tabular}[c]{@{}c@{}}Once during \\ hospitalizations\end{tabular}                                                     & 169        & \cellcolor[HTML]{FED567}149 (88.2\%)                                             \\ \hline
\end{tabular}%
}
    \caption{System usage results, summarized for each form and system section. Cells are highlighted using a continuous red-yellow-green gradient associated with a $0-100\%$ completion scale. Note: the denominator $N$ drops from $274$ to $169$ for forms that are only required following Emergency visits.}\label{tab:usage_tab}
  \end{minipage}%
  \begin{minipage}{.5\linewidth}
    \centering
    \caption{Hospital Web App for Health Personnel, user satisfaction (MARS) survey results, summarized within survey sub-categories across respondents. Cells are colored using a continuous red-yellow-green gradient associated with the 1-5 rating scale values (1=inadequate - 5 = excellent).}\label{tab:MARS_table}
    \resizebox{0.95\linewidth}{!}{%
        \begin{tabular}{|c|c|c|c|
>{\columncolor[HTML]{ABC978}}c |c
>{\columncolor[HTML]{ABC978}}c |}
\hline
\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}MARS \\ Category\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}MARS \\ Subcategory\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{N} & \cellcolor[HTML]{EFEFEF}\textbf{Mean} & \cellcolor[HTML]{EFEFEF}\textbf{Median} & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{IQR}}                       \\ \hline
                                                                                          & \textbf{Graphics}                                                                            & 18                                 & \cellcolor[HTML]{BACB74}3.83          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{EAD36A}3.25} & \cellcolor[HTML]{6CBF85}4.75 \\ \cline{2-7} 
                                                                                          & \textbf{Layout}                                                                              & 18                                 & \cellcolor[HTML]{DBD16D}3.44          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{F2A96D}2}    & 4                            \\ \cline{2-7} 
\multirow{-3}{*}{\textbf{Aesthetics}}                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}Visual \\ Appeal\end{tabular}}                            & 18                                 & \cellcolor[HTML]{C7CD72}3.67          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{ABC978}4}    & 4                            \\ \hline
                                                                                          & \textbf{Fun}                                                                                 & 18                                 & \cellcolor[HTML]{F3AD6C}2.11          & \cellcolor[HTML]{F2A96D}2               & \multicolumn{1}{c|}{\cellcolor[HTML]{E67C73}1}    & \cellcolor[HTML]{FFD666}3    \\ \cline{2-7} 
                                                                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Individual \\ Adaptability\end{tabular}}                  & 18                                 & \cellcolor[HTML]{F0A16E}1.83          & \cellcolor[HTML]{E67C73}1               & \multicolumn{1}{c|}{\cellcolor[HTML]{E67C73}1}    & \cellcolor[HTML]{FFD666}3    \\ \cline{2-7} 
                                                                                          & \textbf{Interactivity}                                                                       & 18                                 & \cellcolor[HTML]{F8BC6A}2.44          & \cellcolor[HTML]{FFD666}3               & \multicolumn{1}{c|}{\cellcolor[HTML]{F2A96D}2}    & \cellcolor[HTML]{FFD666}3    \\ \cline{2-7} 
                                                                                          & \textbf{Interest}                                                                            & 18                                 & \cellcolor[HTML]{CCCE70}3.61          & \cellcolor[HTML]{FFD666}3               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}3}    & \cellcolor[HTML]{6CBF85}4.75 \\ \cline{2-7} 
\multirow{-5}{*}{\textbf{Engagement}}                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}Target \\ Group\end{tabular}}                             & 18                                 & \cellcolor[HTML]{B1CA76}3.94          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{EAD36A}3.25} & 4                            \\ \hline
                                                                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Gestural \\ Design\end{tabular}}                          & 18                                 & \cellcolor[HTML]{E4D26B}3.33          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{F5B46B}2.25} & 4                            \\ \cline{2-7} 
                                                                                          & \textbf{Navigation}                                                                          & 18                                 & \cellcolor[HTML]{A2C879}4.11          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{ABC978}4}    & \cellcolor[HTML]{6CBF85}4.75 \\ \cline{2-7} 
                                                                                          & \textbf{Performance}                                                                         & 18                                 & \cellcolor[HTML]{BACB74}3.83          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{EAD36A}3.25} & 4                            \\ \cline{2-7} 
\multirow{-4}{*}{\textbf{Functionality}}                                                  & \textbf{Usability}                                                                           & 18                                 & \cellcolor[HTML]{D0CF70}3.56          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}3}    & 4                            \\ \hline
                                                                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Description \\ Accuracy\end{tabular}}                     & 18                                 & \cellcolor[HTML]{B5CA76}3.89          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{ABC978}4}    & 4                            \\ \cline{2-7} 
                                                                                          & \textbf{Credibility}                                                                         & 18                                 & \cellcolor[HTML]{94C57D}4.28          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{ABC978}4}    & \cellcolor[HTML]{6CBF85}4.75 \\ \cline{2-7} 
                                                                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Evidence \\ Base\end{tabular}}                            & 10                                 & \cellcolor[HTML]{D5D06F}3.5           & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}3}    & 4                            \\ \cline{2-7} 
                                                                                          & \textbf{Goals}                                                                               & 16                                 & \cellcolor[HTML]{C0CC73}3.75          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}3}    & 4                            \\ \cline{2-7} 
                                                                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Info \\ Quality\end{tabular}}                             & 18                                 & \cellcolor[HTML]{A6C879}4.06          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{ABC978}4}    & \cellcolor[HTML]{6CBF85}4.75 \\ \cline{2-7} 
                                                                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Info \\ Quantity\end{tabular}}                            & 17                                 & \cellcolor[HTML]{B6CB75}3.88          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{ABC978}4}    & 4                            \\ \cline{2-7} 
\multirow{-7}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Information \\ Quality\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Visual Info \\ Quality\end{tabular}}                      & 16                                 & \cellcolor[HTML]{B1CA76}3.94          & 4                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{ABC978}4}    & 4                            \\ \hline
\end{tabular}%
}
\end{minipage} 
\end{table*}
\fi






%old table start
\iffalse
 \begin{table*}
\resizebox{\linewidth}{!}{%
\begin{tabular}{clllll}
\cline{1-3}
\multicolumn{1}{|l|}{\textbf{Interviewee}}                                                                         & \multicolumn{1}{l|}{\textbf{Barrier Description}}                                                                                                                                                                                                                                 & \multicolumn{1}{l|}{\textbf{System Recommendation}}                                                                                                                                                                                                                                                                                                    &  &  &  \\ \cline{1-3}
\multicolumn{1}{|c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Social \\ Worker\end{tabular}}}                    & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(HWA) A limited number of healthcare staff are available for system \\ data collection; medical residents without much system experience \\ were recruited to collect data.\end{tabular}}                                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}More thorough training for system users will help reduce \\ data collection challenges and biases.\end{tabular}}                                                                                                                                                                                        &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers experience fatigue and confusion when filling out \\ forms repeatedly throughout the system.\end{tabular}}                                                                                                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
More user-friendly and instructive design adjustments \\ will be made in future work.
%Eliminate repeated questions across multiple forms in the app. \\ Add additional logic that eliminates cascading questions if \\ certain information is not applicable for the caregiver.
\end{tabular}}                                                                                                 &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers are less interested in participating if they have \\ had a poor experience with physicians (e.g., rude interactions).\end{tabular}}                                                                               & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Healthcare staff will help build positive rapport with \\ families and introduce them to the benefits of the system for their child's \\ wellbeing.\end{tabular}}                                                                                                                                       &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers do not feel they are compensated for their data\\ collection efforts. They also do not observe any direct benefits from \\ using the system.\end{tabular}}                                                        & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}} Future work will include the development of more helpful app \\ features that incentivize use and provide direct benefits to caregivers.\end{tabular}}                                                                                                                                                                          &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers often answer form questions only with respect to \\ the patient and not with respect to themselves (e.g., food security \\ often does not reflect sacrifices that parents make for their children).\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Adding further specifications for certain form questions will \\ ensure better data quality.\end{tabular}}                                                                                                                                                                                              &  &  &  \\ \cline{1-3}
\multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Medical \\ Residents\end{tabular}}}                & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(HWA + FMA) Internet access is often limited both inside and outside \\ the hospital, making it difficult to submit forms.\end{tabular}}                                                                                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Adding modems within the hospital may resolve this issue for\\ the hospital staff.\end{tabular}}                                                                                                                                                                                                        &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers often forget appointments and forget to fill out \\ forms. Others only use the system when they perceive that their child \\ has a possible risk for a complication event.\end{tabular}}                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Additional system features such as reminders and appointment \\ scheduling may assist and incentivize usage. Incorporating a \\ chat bot may also resolve doubts. Caregivers may also benefit \\ from education (via demonstration video) about the importance \\ of the form completion.\end{tabular}} &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(HWA + FMA) Patients and their caregivers often require medical \\ assistance during the journey to the hospital once symptoms of a \\ complication begin.\end{tabular}}                                                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Adding functionalities that allow for communication between \\ caregivers and hospital staff will assist with emergency events \\ (e.g., WhatsApp). An emergency button to notify the hospital \\ about incoming patients would also benefit the care team.\end{tabular}}                               &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(HWA) Some fields are left blank in the emergency forms and are \\ only filled at a later time, which introduces data biases.\end{tabular}}                                                                                        & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Additional training may ensure that the emergency staff \\ completes all fields at the proper time points.\end{tabular}}                                                                                                                                                                                &  &  &  \\ \cline{1-3}
\multicolumn{1}{|c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Participating \\ Caregivers\end{tabular}}}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers expressed that they feel uncomfortable taking \\ vital signs. As a result, they do not collect this information.\end{tabular}}                                                                                    & \multicolumn{1}{l|}{Additional education and training is needed to support.}                                                                                                                                                                                                                                                                           &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers reflect that they did not consider using the app \\ until their child experienced an emergency event.\end{tabular}}                                                                                               & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Additional education and training is needed to support. \\ Additionally, communication between residents and families \\ could be strengthened.\end{tabular}}                                                                                                                                           &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers express uncertainty as to whether or not \\ information they entered has been properly logged in the system.\end{tabular}}                                                                                        & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Need better system design / functionality to confirm that the\\ information was logged properly after form submission, in \\ addition to more app training.\end{tabular}}                                                                                                                               &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{(FMA) Insufficient mobile credit prevents frequent data collection.}                                                                                                                                                                                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
Long-term solutions are needed to address socioeconomic \\ limitations within the populations served. 
%The research team will work on a plan to provide mobile \\ credit funds to families for data collection.
\end{tabular}}                                                                                                                                                                                  &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Most app functionalities are not explained at the time the app\\ is downloaded at the hospital (e.g., some caregivers had no awareness\\ of the mental health pamphlets available within the app).\end{tabular}}             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Better communication and training between social workers \\ and caregivers is needed to close this gap.\end{tabular}}                                                                                                                                                                                   &  &  &  \\ \cline{1-3}
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Non- \\ Participating \\ Caregivers\end{tabular}}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers express that they understand what an emergency \\ event looks like and do not believe the app will provide added support.\end{tabular}}                                                                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Add functionalities that incentivize use of the app beyond \\ emergency event recognition.\end{tabular}}                                                                                                                                                                                                &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Caregivers express that instructions for care at home are not \\ always clear. Written instructions from physicians would be helpful.\end{tabular}}                                                                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Provide functionality that allows physicians to record detailed \\ care instructions so that caregivers can reference them at home.\end{tabular}}                                                                                                                                                       &  &  &  \\ \cline{2-3}
\multicolumn{1}{|c|}{}                                                                                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}(FMA) Some caregivers had no knowledge of the app until late in \\ their child's diagnosis / treatment.\end{tabular}}                                                                                                              & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Provide hospital staff with clarification on patient inclusion \\ criteria for system use.\end{tabular}}                                                                                                                                                                                                &  &  &  \\ \cline{1-3}
\multicolumn{1}{l}{}                                                                                               &                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                                                                                                                                                                        &  &  &  \\
\multicolumn{1}{l}{}                                                                                               &                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                                                                                                                                                                        &  &  & 
\end{tabular}%
}
\caption{Barrier findings and suggested system improvements from unstructured interviews with healthcare staff and caregivers.}
\label{tab:interviews}
\end{table*}
\fi
%old table end
